Loss Terms and Operator Forms of Koopman Autoencoders

Koopman autoencoders are a prevalent architecture in operator learning. But, the loss functions and the form of the operator vary significantly in the literature. This paper presents a fair and systemic study of these options. Furthermore, it introduces novel loss terms.

==> tables/kdv_times.tex <==
\begin{tabular}{lr}
\toprule
option & mean time \\
\midrule
reconstruction & 1.088658 \\
consistency & 0.985603 \\
metric & 0.925739 \\
unitary & 0.922116 \\
determinant & 1.321372 \\
isometry & 0.894227 \\
norm & 1.022971 \\
with & 1.084602 \\
without & 0.887197 \\
\bottomrule
\end{tabular}


==> tables/kdv_top10.tex <==
\begin{tabular}{rlllr}
\toprule
error & accuracy & embedding & operator & dimension \\
\midrule
0.004519 & discounted & reconstruction & unitary & 256 \\
0.004697 & full & consistency & isometry & 256 \\
0.005081 & full & reconstruction & unitary & 256 \\
0.005167 & discounted & consistency & determinant & 128 \\
0.005582 & full & consistency & unitary & 256 \\
0.005680 & full & reconstruction & unitary & 128 \\
0.005806 & discounted & consistency & unitary & 256 \\
0.005870 & discounted & reconstruction & unitary & 128 \\
0.005918 & discounted & consistency & unitary & 128 \\
0.005954 & full & reconstruction & determinant & 256 \\
\bottomrule
\end{tabular}

